Supergiant Temperatures and Linear Radii from Near-Infrared Interferometry

We present angular diameters for 42 luminosity class I stars and 32 luminosity class II stars that have been interferometrically determined with the Palomar Testbed Interferometer. Derived values of radius and effective temperature are established for these objects, and an empirical calibration of these parameters for supergiants will be presented as a functions of spectral type and colors. For the effective temperature versus $(V-K)_0$ color, we find an empirical calibration with a median deviation of $\Delta T = 70$K in the range of $0.7 < (V-K)_0 < 5.1$ for LC I stars; for LC II, the median deviation is $\Delta T = 120$K from $0.4 < (V-K)_0 < 4.3$. Effective temperature as a function of spectral type is also calibrated from these data, but shows significantly more scatter than the $T_{\rm EFF}$ versus $(V-K)_0$ relationship. No deviation of $T_{\rm EFF}$ versus spectral type is seen for these high luminosity objects relative to luminosity class II giants. Directly determined diameters range up to $400 R_\odot$, though are limited by poor distance determinations, which dominate the error estimates. These temperature and radii measures reflect a direct calibration of these parameters for supergiants from empirical means.

==> tab_stardata_LC1.tex <==
\begin{landscape}
\begin{table*}
 \centering
 \begin{minipage}{200mm}
   \caption{Observed and derived supporting parameters for luminosity class I stars.  Spectral type references:
   (1) \citet{1990A&AS...83..225A},
(2) \citet{1958JO.....42..149B},
(3) \citet{1957PASP...69..147B},
(4) \citet{1957POHP....4...11D},
(5) \citet{1961JO.....44..233F},
(6) \citet{1983ApJS...52....7F},
(7) \citet{2001AJ....121.2148G},
(8) \citet{1970ApJ...160.1149H},
(9) \citet{1953ApJ...117..313J},
(10) \citet{1990ApJS...73..769J},
(11) \citet{2001KFNT...17..409K},
(12) \citet{2006yCat.3150....0K},
(13) \citet{1989ApJS...71..245K},
(14) \citet{1958PASP...70..561K},
(15) \citet{1973ARA&A..11...29M},
(16) \citet{1966MNRAS.133..449P},
(17) \citet{1993BICDS..43....5T},
(18) \citet{1961ApJ...134..809Y}\label{table_LC1stars}}
  \begin{tabular}{@{}ccccccccccccccc@{}}
  \hline
{Star ID} &
{points} &
{$\theta_{\rm UD}$} &
{$\chi^2_\nu$} &
{${\overline \delta V^2}$} &
{$\theta_{\rm LD} / \theta_{\rm UD}$} &
{$\theta_{\rm LD}$} &
{$A_V$} &
{$F_{\rm BOL}$} &
{Spectral} &
{Sptype} &
{$V$} &
{$K$} &
{$[12]$} \\
  &
  &
{(mas)} &
 &
 &
 &
{(mas)} &
{(mag)} &
{10$^{-8}$ erg cm$^{-2}$ s$^{-1}$} &
{Type} &
{Ref.} &
{(mag)} &
{(mag)} &
{(mag)}\\
 \hline
HD 4817 & $9/9$ & $2.776 \pm 0.025$ & $0.102$ & $0.006$ & $1.030$ & $2.860 \pm 0.025$ & $0.813 \pm 0.038$ & $52.56 \pm 2.24$ & K5Ib & (12) & 6.04 & $1.50 \pm 0.05$ & 0.90 \\
HD 9366 & $2/2$ & $1.605 \pm 0.106$ & $0.004$ & $0.002$ & $1.026$ & $1.648 \pm 0.109$ & $1.546 \pm 0.043$ & $31.05 \pm 1.16$ & K3Ib & (14) & 6.92 & $2.66 \pm 0.05$ & 1.98 \\
HD 9900 & $2/2$ & $1.579 \pm 0.107$ & $1.368$ & $0.038$ & $1.025$ & $1.618 \pm 0.110$ & $0.899 \pm 0.042$ & $41.47 \pm 2.01$ & K1Ia & (18) & 5.55 & $2.49 \pm 0.09$ & 1.98 \\
HD 11092 & $20/20$ & $2.721 \pm 0.019$ & $0.876$ & $0.020$ & $1.028$ & $2.798 \pm 0.020$ & $1.993 \pm 0.059$ & $82.68 \pm 5.48$ & K5Ia0-a... & (12) & 6.54 & $1.60 \pm 0.06$ & 1.02 \\
HD 12399 & $17/18$ & $1.034 \pm 0.055$ & $0.724$ & $0.027$ & $1.025$ & $1.060 \pm 0.056$ & $2.078 \pm 0.035$ & $17.91 \pm 0.57$ & G5Ia & (3) & 7.53 & $3.89 \pm 0.04$ & 2.81 \\
HD 13658 & $8/9$ & $1.512 \pm 0.073$ & $2.841$ & $0.069$ & $1.029$ & $1.556 \pm 0.075$ & $2.372 \pm 0.047$ & $16.67 \pm 0.59$ & M1Iab & (8) & 8.78 & $3.21 \pm 0.05$ & 2.09 \\
HD 13686 & $8/9$ & $1.538 \pm 0.063$ & $1.685$ & $0.043$ & $1.028$ & $1.581 \pm 0.064$ & $1.272 \pm 0.052$ & $22.49 \pm 1.25$ & K3Ib & (12) & 7.04 & $2.71 \pm 0.09$ & 2.16 \\
HD 14404 & $14/15$ & $2.125 \pm 0.023$ & $1.805$ & $0.036$ & $1.030$ & $2.190 \pm 0.024$ & $1.405 \pm 0.031$ & $28.24 \pm 0.68$ & M2Ib & (12) & 7.78 & $2.36 \pm 0.05$ & 0.86 \\
HD 17958 & $5/5$ & $2.750 \pm 0.032$ & $0.064$ & $0.005$ & $1.026$ & $2.822 \pm 0.033$ & $2.116 \pm 0.043$ & $102.10 \pm 3.97$ & K3Ibvar & (3) & 6.17 & $1.47 \pm 0.05$ & 0.95 \\
HD 18391 & $5/5$ & $1.810 \pm 0.062$ & $3.130$ & $0.055$ & $1.023$ & $1.852 \pm 0.063$ & $2.981 \pm 0.074$ & $74.41 \pm 5.22$ & G0Ia & (12) & 6.86 & $2.42 \pm 0.08$ & 1.54 \\
HD 20902 & $6/6$ & $3.135 \pm 0.029$ & $5.395$ & $0.135$ & $1.017$ & $3.188 \pm 0.030$ & $0.509 \pm 0.025$ & $683.50 \pm 6.84$ & F5Ib & (7) & 1.79 & $0.56 \pm 0.05$ & 0.04 \\
HD 21465 & $5/5$ & $1.833 \pm 0.127$ & $2.064$ & $0.153$ & $1.028$ & $1.884 \pm 0.131$ & $1.465 \pm 0.068$ & $38.07 \pm 2.25$ & K5Iab: & (17) & 7.05 & $2.38 \pm 0.05$ & 1.73 \\
HD 30178 & $11/14$ & $1.807 \pm 0.036$ & $1.407$ & $0.046$ & $1.030$ & $1.862 \pm 0.037$ & $1.130 \pm 0.066$ & $22.88 \pm 1.29$ & M2Ib & (2) & 7.83 & $2.50 \pm 0.09$ & 1.89 \\
HD 31220 & $11/15$ & $2.098 \pm 0.032$ & $0.920$ & $0.031$ & $1.029$ & $2.160 \pm 0.033$ & $1.679 \pm 0.031$ & $37.15 \pm 1.05$ & M0Ib & (4) & 7.40 & $2.20 \pm 0.05$ & 1.52 \\
HD 31910 & $3/3$ & $1.753 \pm 0.059$ & $1.086$ & $0.024$ & $1.020$ & $1.788 \pm 0.060$ & $0.496 \pm 0.020$ & $96.85 \pm 2.18$ & G0Ib & (12) & 4.03 & $2.10 \pm 0.05$ & 1.52 \\
HD 34255 & $3/3$ & $2.585 \pm 0.040$ & $0.605$ & $0.011$ & $1.029$ & $2.661 \pm 0.041$ & $0.562 \pm 0.047$ & $60.62 \pm 2.74$ & K4Iab: & (16) & 5.64 & $1.68 \pm 0.05$ & 1.06 \\
HD 35601 & $3/3$ & $2.817 \pm 0.029$ & $0.805$ & $0.009$ & $1.029$ & $2.900 \pm 0.030$ & $2.326 \pm 0.041$ & $65.57 \pm 2.29$ & M1Ib & (12) & 7.48 & $1.74 \pm 0.08$ & 0.83 \\
HIP 35915 & $3/3$ & $1.943 \pm 0.063$ & $0.034$ & $0.004$ & $1.030$ & $2.002 \pm 0.065$ & $4.728 \pm 0.471$ & $24.70 \pm 15.40$ & M6I-II & (11) & 9.95 & $2.84 \pm 0.10$ & 1.58 \\
HD 37387 & $3/3$ & $1.392 \pm 0.184$ & $0.074$ & $0.020$ & $1.025$ & $1.426 \pm 0.188$ & $2.760 \pm 0.106$ & $35.91 \pm 6.07$ & K1Ib & (8) & 7.52 & $3.02 \pm 0.29$ & 2.25 \\
HD 38247 & $1/1$ & $1.102 \pm 0.429$ & inf & $0.000$ & $1.021$ & $1.126 \pm 0.438$ & $1.812 \pm 0.053$ & $35.69 \pm 2.22$ & G8Iab & (12) & 6.67 & $2.99 \pm 0.25$ & 2.48 \\
HD 44033 & $6/6$ & $2.383 \pm 0.026$ & $0.392$ & $0.025$ & $1.029$ & $2.453 \pm 0.027$ & $0.599 \pm 0.038$ & $43.96 \pm 1.89$ & K3Ib & (5) & 5.67 & $1.76 \pm 0.04$ & 1.19 \\
HD 52005 & $2/2$ & $2.826 \pm 0.113$ & $0.222$ & $0.017$ & $1.030$ & $2.913 \pm 0.116$ & $0.726 \pm 0.025$ & $48.46 \pm 1.22$ & K3Ib & (12) & 5.73 & $1.94 \pm 0.05$ & 1.36 \\
HD 183589 & $23/24$ & $2.720 \pm 0.013$ & $1.565$ & $0.041$ & $1.029$ & $2.800 \pm 0.014$ & $0.974 \pm 0.030$ & $63.91 \pm 2.06$ & K5Ib & (17) & 6.08 & $1.44 \pm 0.05$ & 0.90 \\
HD 186021 & $31/32$ & $1.285 \pm 0.019$ & $1.026$ & $0.030$ & $1.026$ & $1.319 \pm 0.019$ & $1.160 \pm 0.049$ & $23.70 \pm 0.98$ & K0Iab: & (1) & 6.43 & $2.97 \pm 0.26$ & 2.47 \\
HD 187238 & $31/32$ & $1.872 \pm 0.011$ & $1.902$ & $0.031$ & $1.028$ & $1.924 \pm 0.011$ & $1.936 \pm 0.044$ & $41.89 \pm 1.68$ & K3Ia0-a... & (3) & 7.02 & $2.35 \pm 0.05$ & 1.76 \\
HD 193469 & $12/15$ & $2.346 \pm 0.012$ & $1.366$ & $0.020$ & $1.029$ & $2.415 \pm 0.013$ & $0.856 \pm 0.025$ & $42.45 \pm 1.23$ & K5Ib & (3) & 6.35 & $1.81 \pm 0.05$ & 1.29 \\
HD 194093 & $19/22$ & $2.903 \pm 0.008$ & $1.228$ & $0.013$ & $1.018$ & $2.955 \pm 0.008$ & $0.242 \pm 0.012$ & $384.20 \pm 5.22$ & F8Ib & (7) & 2.23 & $0.74 \pm 0.05$ & 0.27 \\
HD 196725 & $28/30$ & $1.705 \pm 0.019$ & $1.018$ & $0.052$ & $1.028$ & $1.753 \pm 0.020$ & $0.151 \pm 0.026$ & $28.92 \pm 0.76$ & K3Ib & (16) & 5.69 & $2.37 \pm 0.05$ & 1.85 \\
HD 197345 & $18/18$ & $2.285 \pm 0.011$ & $2.284$ & $0.024$ & $1.017$ & $2.323 \pm 0.011$ & $0.000 \pm 0.009$ & $816.60 \pm 7.29$ & A2Ia & (9) & 1.25 & $0.90 \pm 0.05$ & 3.37 \\
HD 200576 & $10/10$ & $1.520 \pm 0.045$ & $0.997$ & $0.031$ & $1.029$ & $1.565 \pm 0.046$ & $0.604 \pm 0.099$ & $19.78 \pm 1.59$ & K5Ib & (10) & 6.86 & $2.82 \pm 0.13$ & 2.19 \\
HD 205349 & $14/22$ & $1.539 \pm 0.019$ & $2.203$ & $0.058$ & $1.020$ & $1.569 \pm 0.019$ & $2.251 \pm 0.042$ & $71.29 \pm 2.64$ & K1Ibvar & (3) & 6.27 & $2.19 \pm 0.05$ & 1.56 \\
HD 206859 & $8/9$ & $1.934 \pm 0.028$ & $2.115$ & $0.061$ & $1.021$ & $1.976 \pm 0.028$ & $0.541 \pm 0.017$ & $86.00 \pm 1.74$ & G5Ib & (15) & 4.34 & $1.89 \pm 0.05$ & 1.33 \\
HD 207119 & $14/24$ & $2.252 \pm 0.018$ & $1.186$ & $0.024$ & $1.028$ & $2.315 \pm 0.019$ & $1.177 \pm 0.037$ & $53.13 \pm 2.13$ & K5Ib & (13) & 6.40 & $1.91 \pm 0.05$ & 1.35 \\
HD 207991 & $22/23$ & $1.157 \pm 0.026$ & $1.728$ & $0.039$ & $1.029$ & $1.191 \pm 0.027$ & $0.016 \pm 0.087$ & $12.52 \pm 0.81$ & K5Ib & (13) & 6.88 & $2.93 \pm 0.11$ & 2.50 \\
HD 213306 & $149/152$ & $1.423 \pm 0.007$ & $1.244$ & $0.034$ & $1.018$ & $1.448 \pm 0.007$ & $0.410 \pm 0.022$ & $123.10 \pm 1.95$ & G2Ibvar & (10) & 4.07 & $2.35 \pm 0.05$ & 1.83 \\
HD 216946 & $29/33$ & $3.857 \pm 0.006$ & $2.026$ & $0.013$ & $1.029$ & $3.970 \pm 0.006$ & $0.650 \pm 0.018$ & $119.90 \pm 2.19$ & K5Ibvar & (15) & 4.99 & $0.72 \pm 0.18$ & 0.16 \\
HD 217476 & $27/29$ & $1.224 \pm 0.031$ & $1.109$ & $0.057$ & $1.017$ & $1.245 \pm 0.032$ & $1.889 \pm 0.072$ & $113.80 \pm 7.83$ & G0Ia & (15) & 5.10 & $1.66 \pm 0.05$ & 0.84 \\
HD 224014 & $11/13$ & $2.109 \pm 0.037$ & $1.431$ & $0.052$ & $1.020$ & $2.151 \pm 0.038$ & $1.302 \pm 0.038$ & $130.20 \pm 3.26$ & F8Iavar & (13) & 4.51 & $1.67 \pm 0.05$ & 1.07 \\
HD 236697 & $20/20$ & $1.318 \pm 0.042$ & $0.977$ & $0.033$ & $1.029$ & $1.356 \pm 0.043$ & $1.503 \pm 0.032$ & $13.47 \pm 0.29$ & M2Ib & (12) & 8.69 & $3.24 \pm 0.05$ & 2.49 \\
HD 236915 & $5/5$ & $1.963 \pm 0.092$ & $0.061$ & $0.012$ & $1.030$ & $2.023 \pm 0.094$ & $1.922 \pm 0.058$ & $27.45 \pm 1.28$ & M2Iab & (8) & 8.47 & $2.43 \pm 0.05$ & 1.25 \\
HD 236947 & $10/10$ & $1.596 \pm 0.065$ & $2.551$ & $0.068$ & $1.030$ & $1.644 \pm 0.067$ & $1.737 \pm 0.035$ & $17.52 \pm 0.52$ & M2Ia0-a... & (8) & 8.61 & $2.99 \pm 0.05$ & 2.14 \\
HD 236979 & $5/5$ & $2.734 \pm 0.041$ & $2.516$ & $0.037$ & $1.030$ & $2.818 \pm 0.043$ & $2.146 \pm 0.041$ & $43.15 \pm 1.35$ & M1Iab:var & (10) & 7.99 & $2.03 \pm 0.05$ & -0.34 \\
%\tablerefs{
\hline
\end{tabular}
\end{minipage}
\end{table*}
\end{landscape}






==> tab_stardata_LC2.tex <==
\begin{landscape}
\begin{table*}
 \centering
 \begin{minipage}{200mm}
   \caption{Observed and derived supporting parameters for luminosity class II stars.  Spectral type references:
   (1) \citet{1990A&AS...83..225A},
(2) \citet{1958JO.....42..149B},
(3) \citet{1957PASP...69..147B},
(4) \citet{1957POHP....4...11D},
(5) \citet{1961JO.....44..233F},
(6) \citet{1983ApJS...52....7F},
(7) \citet{2001AJ....121.2148G},
(8) \citet{1970ApJ...160.1149H},
(9) \citet{1953ApJ...117..313J},
(10) \citet{1990ApJS...73..769J},
(11) \citet{2001KFNT...17..409K},
(12) \citet{2006yCat.3150....0K},
(13) \citet{1989ApJS...71..245K},
(14) \citet{1958PASP...70..561K},
(15) \citet{1973ARA&A..11...29M},
(16) \citet{1966MNRAS.133..449P},
(17) \citet{1993BICDS..43....5T},
(18) \citet{1961ApJ...134..809Y}\label{table_LC2stars}.}
  \begin{tabular}{@{}ccccccccccccccc@{}}
  \hline
{Star ID} &
{points} &
{$\theta_{\rm UD}$} &
{$\chi^2_\nu$} &
{${\overline \delta V^2}$} &
{$\theta_{\rm LD} / \theta_{\rm UD}$} &
{$\theta_{\rm LD}$} &
{$A_V$} &
{$F_{\rm BOL}$} &
{Spectral} &
{Sptype} &
{$V$} &
{$K$} &
{$[12]$} \\
  &
  &
{(mas)} &
 &
 &
 &
{(mas)} &
{(mag)} &
{10$^{-8}$ erg cm$^{-2}$ s$^{-1}$} &
{Type} &
{Ref.} &
{(mag)} &
{(mag)} &
{(mag)}\\
 \hline
HD 1613 & $14/14$ & $2.525 \pm 0.026$ & $0.744$ & $0.026$ & $1.029$ & $2.599 \pm 0.026$ & $2.130 \pm 0.065$ & $66.01 \pm 2.79$ & M2II: & (3) & 6.80 & $1.88 \pm 0.22$ & 1.19 \\
HD 3147 & $11/11$ & $1.961 \pm 0.037$ & $0.573$ & $0.024$ & $1.025$ & $2.010 \pm 0.038$ & $2.548 \pm 0.047$ & $64.89 \pm 2.91$ & K2Ib-II & (3) & 6.92 & $2.25 \pm 0.10$ & 1.63 \\
HD 3489 & $9/9$ & $1.375 \pm 0.057$ & $0.987$ & $0.029$ & $1.029$ & $1.415 \pm 0.059$ & $0.643 \pm 0.046$ & $16.13 \pm 0.77$ & K3Ib-II & (3) & 6.77 & $2.79 \pm 0.10$ & 2.33 \\
HD 8701 & $8/8$ & $1.457 \pm 0.064$ & $0.153$ & $0.012$ & $1.021$ & $1.488 \pm 0.065$ & $2.536 \pm 0.073$ & $50.97 \pm 2.80$ & K2II:p & (12) & 6.98 & $2.75 \pm 0.10$ & 2.10 \\
HD 13725 & $6/6$ & $1.545 \pm 0.075$ & $0.475$ & $0.030$ & $1.025$ & $1.584 \pm 0.077$ & $1.845 \pm 0.054$ & $37.01 \pm 2.24$ & K4II & (3) & 7.01 & $2.70 \pm 0.10$ & 2.15 \\
HD 20123 & $5/5$ & $1.585 \pm 0.137$ & $1.472$ & $0.097$ & $1.021$ & $1.619 \pm 0.140$ & $0.914 \pm 0.050$ & $63.03 \pm 2.35$ & G5II & (12) & 5.04 & $2.41 \pm 0.10$ & 1.78 \\
HD 22135 & $5/5$ & $1.493 \pm 0.159$ & $2.373$ & $0.157$ & $1.026$ & $1.533 \pm 0.163$ & $1.783 \pm 0.061$ & $30.12 \pm 2.03$ & K5II & (11) & 7.21 & $2.89 \pm 0.11$ & 2.18 \\
HD 28487 & $4/4$ & $2.808 \pm 0.042$ & $0.501$ & $0.014$ & $1.030$ & $2.893 \pm 0.043$ & $0.467 \pm 0.068$ & $45.04 \pm 2.74$ & M3II & (12) & 6.93 & $1.55 \pm 0.05$ & 0.90 \\
HD 29094 & $19/22$ & $2.627 \pm 0.012$ & $2.589$ & $0.028$ & $1.021$ & $2.684 \pm 0.012$ & $1.211 \pm 0.021$ & $171.70 \pm 3.81$ & G8II & (6) & 4.25 & $1.33 \pm 0.10$ & 0.68 \\
HD 30504 & $15/17$ & $2.727 \pm 0.013$ & $1.732$ & $0.021$ & $1.028$ & $2.803 \pm 0.013$ & $0.258 \pm 0.041$ & $70.80 \pm 3.08$ & K4II & (12) & 4.89 & $1.46 \pm 0.04$ & 0.89 \\
HD 31767 & $4/4$ & $2.598 \pm 0.053$ & $2.874$ & $0.043$ & $1.025$ & $2.662 \pm 0.054$ & $0.811 \pm 0.026$ & $113.90 \pm 2.98$ & K2IIvar & (12) & 4.47 & $1.41 \pm 0.10$ & 0.86 \\
HD 39225 & $3/3$ & $2.387 \pm 0.032$ & $0.157$ & $0.006$ & $1.029$ & $2.457 \pm 0.033$ & $0.910 \pm 0.038$ & $48.18 \pm 2.08$ & M2II: & (12) & 6.04 & $1.82 \pm 0.07$ & 1.00 \\
HD 77912 & $29/36$ & $1.495 \pm 0.013$ & $2.688$ & $0.043$ & $1.020$ & $1.525 \pm 0.013$ & $0.587 \pm 0.048$ & $73.34 \pm 3.98$ & G8Ib-II & (12) & 4.56 & $2.40 \pm 0.09$ & 1.75 \\
HD 84441 & $9/11$ & $2.599 \pm 0.015$ & $1.125$ & $0.016$ & $1.017$ & $2.643 \pm 0.015$ & $1.243 \pm 0.017$ & $453.60 \pm 9.25$ & G0II & (12) & 2.97 & $1.15 \pm 0.10$ & 0.56 \\
HD 159968 & $48/54$ & $2.925 \pm 0.004$ & $1.550$ & $0.013$ & $1.028$ & $3.007 \pm 0.004$ & $1.895 \pm 0.047$ & $84.95 \pm 3.37$ & M1II & (6) & 6.37 & $1.41 \pm 0.10$ & 0.79 \\
HD 163770 & $62/65$ & $3.073 \pm 0.003$ & $1.396$ & $0.008$ & $1.025$ & $3.149 \pm 0.003$ & $0.535 \pm 0.020$ & $154.00 \pm 3.17$ & K1IIvar & (15) & 3.86 & $1.00 \pm 0.19$ & 0.47 \\
HD 180809 & $8/8$ & $2.315 \pm 0.008$ & $2.194$ & $0.014$ & $1.025$ & $2.373 \pm 0.009$ & $0.274 \pm 0.018$ & $81.05 \pm 1.49$ & K0II & (15) & 4.35 & $1.69 \pm 0.10$ & 1.04 \\
HD 181475 & $7/7$ & $2.619 \pm 0.047$ & $0.914$ & $0.043$ & $1.028$ & $2.693 \pm 0.048$ & $2.494 \pm 0.049$ & $75.02 \pm 2.62$ & K5II & (15) & 6.89 & $1.69 \pm 0.05$ & 1.09 \\
HD 185758 & $19/21$ & $1.313 \pm 0.021$ & $1.034$ & $0.042$ & $1.018$ & $1.336 \pm 0.022$ & $1.121 \pm 0.012$ & $111.50 \pm 1.55$ & G0II & (15) & 4.39 & $2.64 \pm 0.10$ & 2.12 \\
HD 185958 & $19/19$ & $1.728 \pm 0.012$ & $1.226$ & $0.037$ & $1.021$ & $1.765 \pm 0.012$ & $0.607 \pm 0.015$ & $81.47 \pm 1.24$ & G8II & (15) & 4.39 & $2.13 \pm 0.10$ & 1.86 \\
HD 191226 & $15/19$ & $1.684 \pm 0.015$ & $1.694$ & $0.031$ & $1.025$ & $1.726 \pm 0.016$ & $2.738 \pm 0.061$ & $49.36 \pm 2.07$ & K2II: & (6) & 7.28 & $2.57 \pm 0.06$ & 2.03 \\
HD 193092 & $8/14$ & $2.666 \pm 0.018$ & $0.557$ & $0.015$ & $1.028$ & $2.741 \pm 0.018$ & $0.724 \pm 0.036$ & $76.77 \pm 3.17$ & K5II & (15) & 5.27 & $1.45 \pm 0.03$ & 0.99 \\
HD 193217 & $3/3$ & $1.771 \pm 0.104$ & $3.230$ & $0.071$ & $1.029$ & $1.823 \pm 0.107$ & $0.609 \pm 0.037$ & $26.25 \pm 1.12$ & K4II: & (13) & 6.32 & $2.48 \pm 0.08$ & 2.02 \\
HD 196819 & $5/5$ & $1.177 \pm 0.108$ & $1.578$ & $0.048$ & $1.026$ & $1.208 \pm 0.111$ & $1.358 \pm 0.039$ & $16.70 \pm 0.77$ & K3II & (13) & 7.52 & $3.25 \pm 0.32$ &  \\
HD 199098 & $5/5$ & $1.026 \pm 0.114$ & $1.004$ & $0.036$ & $1.019$ & $1.046 \pm 0.117$ & $0.789 \pm 0.045$ & $38.80 \pm 1.92$ & K0II & (6) & 5.48 & $3.00 \pm 0.29$ &  \\
HD 213179 & $6/6$ & $1.408 \pm 0.037$ & $0.155$ & $0.013$ & $1.028$ & $1.448 \pm 0.038$ & $0.191 \pm 0.086$ & $19.62 \pm 1.72$ & K2II & (18) & 5.79 & $2.98 \pm 0.25$ & 2.45 \\
HD 217673 & $9/9$ & $1.093 \pm 0.053$ & $0.750$ & $0.031$ & $1.023$ & $1.118 \pm 0.054$ & $0.864 \pm 0.040$ & $24.32 \pm 1.05$ & K2II & (13) & 6.24 & $2.82 \pm 0.12$ & 2.22 \\
HD 218356 & $43/49$ & $2.200 \pm 0.008$ & $1.918$ & $0.056$ & $1.028$ & $2.262 \pm 0.008$ & $0.141 \pm 0.028$ & $48.84 \pm 1.48$ & K0IIp & (13) & 4.76 & $1.79 \pm 0.10$ & 1.22 \\
HD 220369 & $8/9$ & $2.136 \pm 0.030$ & $2.720$ & $0.044$ & $1.025$ & $2.189 \pm 0.031$ & $0.942 \pm 0.043$ & $68.82 \pm 3.01$ & K3II & (6) & 5.56 & $1.72 \pm 0.06$ & 1.17 \\
HD 223173 & $10/12$ & $2.262 \pm 0.029$ & $1.603$ & $0.045$ & $1.028$ & $2.326 \pm 0.029$ & $0.690 \pm 0.046$ & $56.36 \pm 2.82$ & K3II & (15) & 5.55 & $1.89 \pm 0.05$ & 1.29 \\
HD 223332 & $25/28$ & $1.122 \pm 0.022$ & $1.555$ & $0.115$ & $1.028$ & $1.153 \pm 0.022$ & $0.638 \pm 0.064$ & $13.36 \pm 0.91$ & K5II & (6) & 7.03 & $3.58 \pm 0.31$ & 2.74 \\
HD 334750 & $3/3$ & $2.250 \pm 0.036$ & $3.770$ & $0.040$ & $1.030$ & $2.319 \pm 0.038$ & $1.955 \pm 0.103$ & $22.86 \pm 2.64$ & M5II & (10) & 9.13 & $2.33 \pm 0.08$ & 1.53 \\
\hline
\end{tabular}
\end{minipage}
\end{table*}
\end{landscape}





